Architectural Implications of Embedding Dimension during GCN on CPU and GPU

Graph Neural Networks (GNNs) are a class of neural networks designed to extract information from the graphical structure of data. Graph Convolutional Networks (GCNs) are a widely used type of GNN for transductive graph learning problems which apply convolution to learn information from graphs. GCN is a challenging algorithm from an architecture perspective due to inherent sparsity, low data reuse, and massive memory capacity requirements. Traditional neural algorithms exploit the high compute capacity of GPUs to achieve high performance for both inference and training. The architectural decision to use a GPU for GCN inference is a question explored in this work. GCN on both CPU and GPU was characterized in order to better understand the implications of graph size, embedding dimension, and sampling on performance.

==> text/layerwise_sampling.tex <==
\begin{algorithm}
\caption{Layer-Wise Neighborhood-Sampling}\label{alg:layer-wise}
\begin{algorithmic}[1]

\Statex{
    \textbf{Input:} 
    Subgraph loader $S$, 
    feature matrix $H_{in}\in \mathbb{R}^{|V|\times K}$,
    gcn layer list $G$
}
\Statex{
    \textbf{Output:} 
    $H_{out}\in \mathbb{R}^{|V|\times K}$
}
\Procedure{Layer-Wise}{}

\ForEach{layer $l\in G$ }

\State {
    $x_{int} = [ \ ]$
}

\ForEach {
    $batch, nid, adj \in S$
}

\If{
    $e \ge row[u+1]$} \Comment{\small{\emph{Vertex completed}}
}
\State{
    $H_{out}[u, :] \leftarrow H_{out}[u, :] + B[:]$ \Comment{\small{\emph{Atomic write}}}
}
\State{
    $u\leftarrow u+1,\ B[:] \leftarrow 0$
}
\EndIf

\State{$v\leftarrow col[e]$ \Comment{\small{\emph{Neighbor vertex}}}}
\State {$B[:] \ {\leftarrow}\ B[:] +  \Tilde{\mA}[u,v]*H_{in}[v, :]$\Comment{\small{\emph{Accumulate}}}}\label{algo:line:accum}

\EndForEach
% \State{$H_{out}[v, :] = H_{op}[v, :] + B[:]$}
\EndParForEach
\EndProcedure
\end{algorithmic}
\end{algorithm}


==> text/related_work.tex <==
\section{Related Work}

talks about GPU performance during inference and training - page 187 figures 36 a/b has batched inference on GPU where most of the time is spent either sampling or data transfer to GPU \cite{wang_empirical_2021}.

Figure 7 shows most of the time is spent sampling and data loading on GPU as well \cite{zhang_pcgraph_2021}.


Row Parallel Edge parallel Merge parallel \cite{yang_design_2018}


